Decomposable Non-Smooth Convex Optimization with Nearly-Linear Gradient Oracle Complexity

Many fundamental problems in machine learning can be formulated by the convex program \[ \min_{\theta\in R^d}\ \sum_{i=1}^{n}f_{i}(\theta), \] where each $f_i$ is a convex, Lipschitz function supported on a subset of $d_i$ coordinates of $\theta$. One common approach to this problem, exemplified by stochastic gradient descent, involves sampling one $f_i$ term at every iteration to make progress. This approach crucially relies on a notion of uniformity across the $f_i$'s, formally captured by their condition number. In this work, we give an algorithm that minimizes the above convex formulation to $\epsilon$-accuracy in $\widetilde{O}(\sum_{i=1}^n d_i \log (1 /\epsilon))$ gradient computations, with no assumptions on the condition number. The previous best algorithm independent of the condition number is the standard cutting plane method, which requires $O(nd \log (1/\epsilon))$ gradient computations. As a corollary, we improve upon the evaluation oracle complexity for decomposable submodular minimization by Axiotis et al. (ICML 2021). Our main technical contribution is an adaptive procedure to select an $f_i$ term at every iteration via a novel combination of cutting-plane and interior-point methods.

==> preamble.tex <==
\floatstyle{ruled}
\newfloat{algorithm}{tbp}{loa}
\providecommand{\algorithmname}{Algorithm}
\floatname{algorithm}{\protect\algorithmname}

\makeatletter

\theoremstyle{plain}
\newtheorem{thm}{\protect\theoremname}
\theoremstyle{definition}
\newtheorem{defn}[thm]{\protect\definitionname}
\theoremstyle{conjecture}
\newtheorem{conj}[thm]{\protect\conjecturename}

\theoremstyle{plain}
\newtheorem{prob}[thm]{\protect\problemname}

\theoremstyle{plain}
\newtheorem{lem}[thm]{\protect\lemmaname}

\theoremstyle{plain}
\newtheorem{assumption}[thm]{\protect\assumptionname}

\theoremstyle{plain}
\newtheorem{cor}[thm]{\protect\corollaryname}
\theoremstyle{plain}
\newtheorem{prop}[thm]{\protect\propositionname}
\theoremstyle{remark}
\newtheorem{rem}[thm]{\protect\remarkname}

\theoremstyle{fact}
\newtheorem{fact}[thm]{\protect\factname}

\usepackage[most]{tcolorbox}
\usepackage{setspace}
\usepackage{enumitem}
\usepackage{caption}
\captionsetup{font=small}
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}} 
\usepackage{color,calc}
\definecolor{shade}{gray}{0.8}
\newenvironment{myshadedbox}[1][]        {
                \footnotesize\normalfont\ttfamily\raggedright
        \setlength{\rightmargin}{\leftmargin}
        \setlength{\itemsep}{-12pt}
        \setlength{\parsep}{20pt}
        \begin{lrbox}{\@tempboxa}        \begin{minipage}{\linewidth-2\fboxsep}
        }        {
        \end{minipage}        \end{lrbox}        \fcolorbox{black}{shade}{\usebox{\@tempboxa}}\newline\newline
        }\usepackage{algorithm, algorithmicx, algpseudocode}
\usepackage[margin=1in]{geometry}
\usepackage{hyperref}
\usepackage{tikz}
\usepackage{amsthm}

\newcommand\blfootnotea[1]{  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}  \endgroup
}

\newcommand{\declarecolor}[2]{\definecolor{#1}{RGB}{#2}\expandafter\newcommand\csname #1\endcsname[1]{\textcolor{#1}{##1}}}
\declarecolor{White}{255, 255, 255}
\declarecolor{Black}{0, 0, 0}
\declarecolor{LightGray}{216, 216, 216}
\declarecolor{Gray}{127, 127, 127}
\declarecolor{Orange}{237, 125, 49}
\declarecolor{LightOrange}{251,229, 214}
\declarecolor{Yellow}{255, 192, 0}
\declarecolor{LightYellow}{255, 242, 200}
\declarecolor{Blue}{91, 155, 213}
\declarecolor{LightBlue}{222, 235, 247}
\declarecolor{Green}{112, 173, 71}
\declarecolor{LightGreen}{226, 240, 217}
\declarecolor{Navy}{68, 114, 196}
\declarecolor{LightNavy}{218, 227, 243}

\numberwithin{equation}{section}
\numberwithin{thm}{section}

\hypersetup{
	colorlinks=true,
	pdfpagemode=UseNone,
	citecolor=Green,
	linkcolor=Navy,
	urlcolor=Black
}

\usepackage{booktabs, makecell}
\usepackage{graphicx}
\usepackage{babel}
\usepackage{thmtools, thm-restate}


\providecommand{\corollaryname}{Corollary}
\providecommand{\definitionname}{Definition}
\providecommand{\problemname}{Problem}
\providecommand{\lemmaname}{Lemma}
\providecommand{\propositionname}{Proposition}
\providecommand{\remarkname}{Remark}
\providecommand{\theoremname}{Theorem}
\providecommand{\conjecturename}{Conjecture}
\providecommand{\assumptionname}{Assumption}
\providecommand{\factname}{Fact}

\newcommand{\todo}[1]{\textcolor{blue}{TODO: #1}}
\newcommand{\Sally}[1]{\textcolor{magenta}{Sally: #1}}
\newcommand{\Guanghao}[1]{\textcolor{Orange}{Guanghao: #1}}
\newcommand{\swati}[1]{\textcolor{Green}{SP: #1}}
\newcommand{\haotian}[1]{\textcolor{red}{Haotian: #1}}

\usepackage[capitalize, nameinlink]{cleveref}

\crefname{prob}{Problem}{Problems}
\crefname{conj}{Conjecture}{Conjectures}
\crefname{sec}{Section}{Sections}
\crefname{assumption}{Assumption}{Assumptions}
\crefformat{none}{(#2#1#3)}
\crefname{equation}{Equation}{Equations}
\crefname{lem}{Lemma}{Lemmas}
\crefname{rem}{Remark}{Remarks}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{prop}{Proposition}{Propositions}
\crefname{defn}{Definition}{Definitions}
\crefname{cor}{Corollary}{Corollaries}
\crefname{ineq}{Inequality}{Inequalities}
\crefname{fact}{Fact}{Facts}
\crefname{assumption}{Assumption}{Assumptions}
\creflabelformat{ineq}{#2{\upshape(#1)}#3} 
\crefalias{thm}{theorem}
\let\cref\cref

\makeatother
\global\long\def\vx{\mathbf{x}}\global\long\def\vtheta{\mathbf{\theta}}\global\long\def\vc{\mathbf{c}}\global\long\def\vb{\mathbf{b}}\global\long\def\ovx{\overline{\mathbf{x}}} 
\global\long\def\ma{\mathbf{A}}\global\long\def\vxi{\vx_{i}}\global\long\def\vthetai{\vtheta_{i}}\global\long\def\vxos{\vx_{\textrm{out}}^{\star}}\global\long\def\vxosi{\vx_{\textrm{out,}i}^{\star}}\global\long\def\vxoutput{\vx_{\textrm{output}}}\global\long\def\vxin{\vx_{\textrm{in}}}\global\long\def\vv{\mathbf{v}}\global\long\def\vw{\mathbf{w}}\global\long\def\vz{\mathbf{z}}\global\long\def\vzi{\vz_{i}}\global\long\def\vy{\mathbf{y}}\global\long\def\vxt{\vx_{t}}\global\long\def\vu{\mathbf{u}}\global\long\def\ve{\mathbf{e}}\global\long\def\deltaX{\delta_{\vx}}\global\long\def\deltaXi{\delta_{\vx,i}}
\global\long\def\ki{\mathcal{K}_{i}}\global\long\def\kini{\mathcal{K}_{\textrm{in,}i}}\global\long\def\kout{\mathcal{K}_{\textrm{out}}}\global\long\def\kouti{\mathcal{K}_{\mathrm{out,}i}}\global\long\def\kcal{\mathcal{K}}\global\long\def\koutnew{\mathcal{K}_{\textrm{out,new}}}\global\long\def\ball{\mathcal{B}}\global\long\def\oi{\mathcal{O}_{i}}\global\long\def\hi{\mathcal{H}_{i}}\global\long\def\conv{\mathrm{conv}}\global\long\def\h{\mathcal{H}}\global\long\def\vol{\mathrm{vol}}\global\long\def\koutbar{\overline{\mathcal{K}}_{\textrm{out}}}\global\long\def\kinbar{\overline{\mathcal{K}}_{\textrm{in}}}
\global\long\def\kouthat{\widehat{\mathcal{K}}_{\textrm{out}}}\global\long\def\kinhat{\widehat{\mathcal{K}}_{\textrm{in}}}

\global\long\def\iter{\mathcal{T}}\global\long\def\kin{\mathcal{K}_{\textrm{in}}}\global\long\def\pin{\mathcal{P}_{\textrm{in}}}\global\long\def\kh{\mathcal{K}_{\h}}
\global\long\def\R{\mathbb{R}}\global\long\def\inprod#1#2{\langle#1,#2\rangle}\global\long\def\E{\mathbb{E}}\global\long\def\norm#1{\|#1\|}\global\long\def\defeq{\stackrel{\textrm{def}}{=}}\global\long\def\Rn{\mathbb{R}^{n}}
\global\long\def\barrini{\psi_{\textrm{in,}i}}\global\long\def\barrin{\psi_{\textrm{in}}}\global\long\def\barrouti{\psi_{\textrm{out,}i}}\global\long\def\barrout{\psi_{\textrm{out}}}\global\long\def\barr{\psi}\global\long\def\barrUniK{\psi_{\mathcal{K}}}\global\long\def\barrUniKNew{\psi_{\mathcal{K},\textrm{new}}}
\global\long\def\pot{\Phi}\global\long\def\potinit{\pot_{\textrm{init}}}
\global\long\def\potend{\pot_{\textrm{end}}}

\global\long\def\potipm{\Phi^{\textrm{(x)}}}\global\long\def\Et#1#2{\xi_{#2}^{#1}}\global\long\def\potkout{\Phi_{-t\vc}^{\textrm{(out)}}(\Omega)}\global\long\def\potkoutnew{\Phi_{-t\vc}^{\textrm{(out)}}(\Omega_{\textrm{new}})}\global\long\def\pott{\Phi_{\vx}^{(\textrm{t)}}(t)}\global\long\def\pottnew{\Phi_{\vx}^{\textrm{(t)}}(t_{\textrm{new}})}\global\long\def\potkin{\Phi_{\vx}^{\textrm{(in)}}(\kini)}\global\long\def\potkinnew{\Phi_{\vx}^{\textrm{(in)}}(\mathcal{K}_{\textrm{in},i,\textrm{new}})}\global\long\def\potnew{\Phi^{\textrm{(new)}}}
\global\long\def\nt{\mathcal{N}_{\textrm{t}}}
\global\long\def\nx{\mathcal{N}_{\vx}}
\global\long\def\nout{\mathcal{N}_{\textrm{out}}}
\global\long\def\nin{\mathcal{N}_{\textrm{in}}}
\global\long\def\nn{\mathcal{N}_{\textrm{total}}}
\global\long\def\nsep{\mathcal{N}_{\textrm{sep}}}
\global\long\def\vh{\mathbf{h}}
\global\long\def\tinit{t_{\textrm{init}}}
\global\long\def\tend{t_{\textrm{end}}}


\newcommand{\poly}{\mathrm{poly}}
\newcommand{\polylog}{\mathrm{polylog}}

\newcommand{\EO}{\mathsf{EO}}

